A Historical Account of My Early Research Interests

This paper presents a brief account of some of the my early research interests. This historical account starts from my laurea thesis on Signal Theory and my master thesis on Computation Theory. It recalls some results in Combinatory Logic and Term Rewriting Systems. Some other results concern Program Transformation, Parallel Computation, Theory of Concurrency, and Proof of Program Properties. My early research activity has been mainly done in cooperation with Andrzej Skowron, Anna Labella, and Maurizio Proietti.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{L. Fribourg and M. Heizmann (Eds.): VPT/HCVS 2020\\
EPTCS 320, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.320.1}{10.4204/EPTCS.320.1}}

